Sample Complexity of Asynchronous Q-Learning: Sharper Analysis and Variance Reduction

Asynchronous Q-learning aims to learn the optimal action-value function (or Q-function) of a Markov decision process (MDP), based on a single trajectory of Markovian samples induced by a behavior policy. Focusing on a $\gamma$-discounted MDP with state space $\mathcal{S}$ and action space $\mathcal{A}$, we demonstrate that the $\ell_{\infty}$-based sample complexity of classical asynchronous Q-learning --- namely, the number of samples needed to yield an entrywise $\varepsilon$-accurate estimate of the Q-function --- is at most on the order of $\frac{1}{\mu_{\min}(1-\gamma)^5\varepsilon^2}+ \frac{t_{mix}}{\mu_{\min}(1-\gamma)}$ up to some logarithmic factor, provided that a proper constant learning rate is adopted. Here, $t_{mix}$ and $\mu_{\min}$ denote respectively the mixing time and the minimum state-action occupancy probability of the sample trajectory. The first term of this bound matches the sample complexity in the synchronous case with independent samples drawn from the stationary distribution of the trajectory. The second term reflects the cost taken for the empirical distribution of the Markovian trajectory to reach a steady state, which is incurred at the very beginning and becomes amortized as the algorithm runs. Encouragingly, the above bound improves upon the state-of-the-art result \cite{qu2020finite} by a factor of at least $|\mathcal{S}||\mathcal{A}|$ for all scenarios, and by a factor of at least $t_{mix}|\mathcal{S}||\mathcal{A}|$ for any sufficiently small accuracy level $\varepsilon$. Further, we demonstrate that the scaling on the effective horizon $\frac{1}{1-\gamma}$ can be improved by means of variance reduction.

==> main-results.tex <==
\section{Main results}
\label{sec:main-results}


% \newcommand{\Qstar}{Q^\star}



\subsection{Theoretical Guarantees for Asynchronous Q-Learning }
With the above parameters in place, we are in a position to present our main theory regarding the (non-asymptotic) sample complexity of asynchronous Q-learning.
%
\begin{theorem}[Asynchronous Q-learning]
	\label{thm:main-asyn-Q-learning}
	Consider the asynchronous Q-learning algorithm~\eqref{eqn:q-learning}.
	There exist some universal constants $c_0,c_1>0$ such that for any $0<\delta<1$ and $0<\varepsilon \leq \frac{1}{1-\gamma}$,  one has
%
	\begin{align*}
		\forall (s,a)\in \cS\times \cA: \qquad |Q_T (s,a) - Q^\star(s,a)| \leq \varepsilon
	\end{align*}
%
	with probability at least $1-\delta$, provided that the iteration number $T$ and the learning rates $\eta_t \equiv \eta $ obey
	\begin{subequations}
	%
	\begin{align}
	\label{eqn:numbersteps}
		T & =\frac{c_{0}}{\mu_{\min}}\left\{ \frac{1}{(1-\gamma)^{5}\varepsilon^{2}}+\frac{\tmix}{1-\gamma}\right\} 
		\log\Big( \frac{|\mathcal{S}||\mathcal{A}|T}{\delta} \Big) \log \Big(\frac{1}{(1-\gamma)^2\varepsilon} \Big),\\
		\eta & =\frac{c_{1}}{\log\big(\frac{|\mathcal{S}||\mathcal{A}|T}{\delta}\big)}\min\left\{ \frac{(1-\gamma)^{4}\varepsilon^{2}}{\gamma^{2}},~\frac{1}{\tmix}\right\} .
	\end{align}
	%
	\end{subequations}
\end{theorem}


We provide an immediate corollary that provides the first non-asymptotic $\ell_\infty$ guarantee to asynchronous TD learning over Markovian data by taking the action space as a singleton. 
\begin{corollary}[Asynchronous TD learning] \label{corollary:asynTD}
	Consider the TD learning algorithm~\eqref{eqn:td-learning}.
	There exist some universal constants $c_0,c_1>0$ such that for any $0<\delta<1$ and $0<\varepsilon \leq \frac{1}{1-\gamma}$,  one has
%
	\begin{align*}
		\forall (s,a)\in \cS\times \cA: \qquad |V_T (s) - V^\pi (s)| \leq \varepsilon
	\end{align*}
%
	with probability at least $1-\delta$, provided that the iteration number $T$ and the learning rates $\eta_t \equiv \eta $ obey
	\begin{subequations}
	%
	\begin{align}
	\label{eqn:numbersteps}
		T & =\frac{c_{0}}{\mu_{\min}}\left\{ \frac{1}{(1-\gamma)^{5}\varepsilon^{2}}+\frac{\tmix}{1-\gamma}\right\} 
		\log\Big( \frac{|\mathcal{S} | T}{\delta} \Big) \log \Big(\frac{1}{(1-\gamma)^2\varepsilon} \Big),\\
		\eta & =\frac{c_{1}}{\log\big(\frac{|\mathcal{S}| T}{\delta}\big)}\min\left\{ \frac{(1-\gamma)^{4}\varepsilon^{2}}{\gamma^{2}},~\frac{1}{\tmix}\right\} .
	\end{align}
	%
	\end{subequations}
\end{corollary}

 
	

	% and $t \geq \frac{\log(\frac{|\cirS||\A|\tepoch}{\delta(1-\gamma)})}{(1-\gamma)^5\epsilon^2}\tepoch $
	% and the step size 
	% $\eta_t \equiv \eta = \frac{(1-\gamma)^4\epsilon^2}{\log(\frac{|\cirS||\A|\tepoch}{\delta(1-\gamma)})}$, for all state-action pair $(s,a) \in \cirS \times \A$, 
	% holds with .

\subsection{Theoretical Guarantees for Asynchronous Variance-Reduced Q-Learning}


\begin{theorem}[Asynchronous Variance-Reduced Q-learning]
	\label{thm:main-asyn-VR-Q-learning}
	Consider the asynchronous variance-reduced Q-learning algorithm in \eqref{eqn:vr-q-learning-epoch}.
	There exist some universal constants $c_0,c_1>0$ such that for any $0<\delta<1$ and $0<\varepsilon \leq 1$,  one has
%
	\begin{align*}
		\forall (s,a)\in \cS\times \cA: \qquad |Q_T (s,a) - Q^\star(s,a)| \leq \varepsilon
	\end{align*}
%
	with probability at least $1-\delta$, provided that the iteration number $T$ and the learning rates $\eta_t \equiv \eta $ obey \yjc{to be updated with more parameters.}
	\begin{subequations}
	%
	\begin{align}
	\label{eqn:numbersteps}
		T & =\frac{c_{0}}{\mu_{\min}}\left\{ \frac{1}{(1-\gamma)^{3}\varepsilon^{2}}+\frac{\tmix}{1-\gamma}\right\} 
		\log\Big( \frac{|\mathcal{S}||\mathcal{A}|T}{\delta} \Big) \log \Big(\frac{1}{(1-\gamma)^2\varepsilon} \Big),\\
		\eta & =\frac{c_{1}}{\log\big(\frac{|\mathcal{S}||\mathcal{A}|T}{\delta}\big)}\min\left\{ \frac{(1-\gamma)^{2} }{\gamma^{2}},~\frac{1}{\tmix}\right\} .
	\end{align}
	%
	\end{subequations}
\end{theorem}

Again, it is possible to state a similar results for asynchronous variance-reduced TD learning by reducing the action space to a singleton.  
This theorem generalizes the analysis in \cite{wainwright2019variance} for Q-learning, as well as the analysis in \cite{khamaru2020temporal} for TD learning to the asynchronous setting using a constant step size.


==> matrix_notation.tex <==
\subsection{Matrix notation and Bellman equations} 

It is convenient to present our proof based on some matrix notation for MDPs.  Denoting by $\bm{e}_1,\cdots,\bm{e}_{|\mathcal{S}|}\in \mathbb{R}^{|\mathcal{S}|}$ the standard basis vectors, we can define: 
%
\begin{itemize}
	\item $\bm{r} \in \mathbb{R}^{|\mathcal{S}||\mathcal{A}|}$: a vector representing the reward function $r$ (so that $r_{(s,a)} =r(s,a)$ for all $(s,a)\in \cS\times \cA$). 
	\item $\bm{V}^{\pi} \in \mathbb{R}^{|\mathcal{S}|}$: a vector representing the value function $V^{\pi}$ (so that ${V}^{\pi}_s = {V}^{\pi}(s)$ for all $s\in \cS$).
	\item $\bm{Q}^{\pi} \in \mathbb{R}^{|\mathcal{S}||\mathcal{A}|}$: a vector representing the Q-function $Q^{\pi}$ (so that ${Q}^{\pi}_{(s,a)} = {Q}^{\pi}(s,a)$ for all $(s,a)\in \cS\times \cA$).
	\item  $\bm{V}^{\star} \in \mathbb{R}^{|\mathcal{S}|}$ and $\bm{Q}^{\star} \in \mathbb{R}^{|\mathcal{S}||\mathcal{A}|}$: representing the optimal value function $V^{\star}$ and optimal Q-function $Q^{\star}$.
	\item $\bm{P}\in \mathbb{R}^{|\cS||\cA|\times |\cS|}$: a matrix representing the probability transition kernel $P$, where the $(s,a)$-th row of $\bm{P}$ is a probability vector representing $P(\cdot|s,a)$.  
	Denote $\bm P_{s,a}$ as the $(s,a)$-th row of the transition matrix $\bm P$. 
	\item $\bm{\Pi}^{\pi} \in \{0,1\}^{|\cS| \times |\cS||\cA|}$: a projection matrix associated with a given policy $\pi$ taking the following form
\begin{align}
\label{eqn:bigpi}
	\bPi^{\pi} = {\scriptsize
	\begin{pmatrix}
		\e_{\pi(1)}^\top &            &  \\
		           & \e_{\pi(2)}^\top &  \\
		           &            & \ddots \\	
		           &            &         & \e_{\pi(|\cS|)}^\top
	\end{pmatrix}  }.
\end{align}
	\item $\bm{P}^{\pi} \in \mathbb{R}^{|\cS| |\cA|\times |\cS| |\cA|}$ and $\bm{P}_{\pi} \in \mathbb{R}^{|\cS| \times |\cS| }$: two {\em square} probability transition matrices induced by the policy $\pi$ over the state-action pairs and the states respectively, defined by
		%
	\begin{equation}
	\label{eqn:ppivq}
		\Pq \defn \bP \bPi^{\pi} \qquad \text{and} \qquad \Pv \defn \bPi^{\pi} \bP .
	\end{equation}

\item $\bm{r}_{\pi} \in \mathbb{R}^{|\cS|}$: a reward vector restricted to the actions chosen by the policy $\pi$, namely,  $r_{\pi}(s) = r(s,\pi(s))$ for all $s\in \cS$ (or simply, $\bm{r}_{\pi}=\bm{\Pi}^{\pi}\bm{r}$). 
\end{itemize}

% Let us represent the value function $V^{\pi}$ (resp.~$V^{\star}$) by a vector $\bm{V}^{\pi}\in \mathbb{R}^{|\mathcal{S}|}$ (resp.~$\bm{V}^{\star}\in \mathbb{R}^{|\mathcal{S}|}$), and the action-value function $Q^{\pi}$ (resp.~$Q^{\star}$) be a vector $\bm{Q}^{\pi}\in \mathbb{R}^{|\cS||\cA|}$ (resp.~$\bm{Q}^{\star}\in \mathbb{R}^{|\cS||\cA|}$). Let $\bm{r}$ be the reward vector of length $|\cS||\cA|$. 

% Let $\bm{P}$ be a matrix of size $|\cS| |\cA| \times |\cS|$ where each row corresponds to a state-action pair $(s,a)$, each column corresponds to a state $s^{\prime}$, and each entry corresponds to the probability $P(s^{\prime}|s,a)$. 
% Let $\bm{\Pi}$ be a binary matrix of size $|\cS| \times |\cA|$ denote the policy $\pi$, where the $(s,a)$ entry is $1$ if and only if $\pi(s) = a$, and $0$ otherwise. We have


% where  $ \e_{\pi(i)}^\top = (0,\ldots, 1,\ldots,0) \in \real^{|\mathcal{S}|}$ is the standard basis vector with $1$ at the $\pi(i)$th entry.

% We also define the matrix $\bm{P}^{\pi}$ of size $|\cS| |\cA| \times |\cS||\cA|$ to be the transition matrix on state-action pairs induced by a policy $\pi$, where the $(s,a)\times(s^\prime, a^\prime)$ entry equals $P(s^{\prime}|s,a)$  if and only if $a^\prime = \pi (s^\prime)$, and $0$ otherwise. Using matrix notations, we have
% \begin{align}
% \label{eqn:ppiq}
% 	\Pq \defn \bP \bPi^{\pi} ,
% \end{align}
% where
% \begin{align}
% \label{eqn:bigpi}
% 	\bPi^{\pi} = 
% 	\begin{pmatrix}
% 		\e_{\pi(1)}^\top &            &  \\
 %		           & \e_{\pi(2)}^\top &  \\
% 		           &            & \ddots \\	
% 		           &            &         & \e_{\pi(|\cS|)}^\top
% 	\end{pmatrix} \in \{0,1\}^{|\cS|\times |\cS||\cA|}.
% \end{align}

% Furthermore, we define the matrix $\Pv$ of size $|\cS|\times |\cS|$ as the transition matrix on states induced by a policy $\pi$:


\noindent Armed with the above matrix notation, we can write, for any policy $\pi$, the {\em Bellman consistency equation} as
%
\begin{equation} \label{eq:bellman_consistency_q}
\bm{Q}^{\pi}  = \bm{r} + \gamma \bm{P} \bm{V}^{\pi} = \bm{r} + \gamma \Pq  \bm{Q}^{\pi} ,
\end{equation}
%
which implies that
%
\begin{align}
	& \bm{Q}^{\pi} = (\bm{I} -  \gamma \Pq)^{-1} \bm{r} ; \\
%
	\bm{V}^{\pi} =  \bm{r}_{\pi} + \gamma \Pv & \bm{V}^{\pi} 
	\qquad \text{and} \qquad
	\bm{V}^{\pi}  = (\bm{I} -  \gamma \Pv)^{-1}    \bm{r}_{\pi} .  \label{eq:bellman_consistency_v}
\end{align}
%
%where $\bm{r}_{\pi} =  \bPi^{\pi}  \bm{r}$ is the $|\cS|$-dimensional state reward vector induced by $\pi$ and $\bm{r}$.
For a vector $\bm{V}=[V_i]_{1\leq i\leq |\mathcal{S}|}\in\real^{|\cS|}$, we define the vector $\Var_{\bP}(\bm{V}) \in \real^{|\cS||\cA|}$ whose entries are given by 
%
\begin{align*}
	\forall (s,a)\in \cS \times \cA, \qquad \big[\Var_{\bP}(\bm{V})\big]_{(s,a)}: = \sum_{s'\in \cS} P(s'| s,a) V_{s'}^2 
	-  \Big( \sum_{s'\in \cS}P(s'| s,a) V_{s'} \Big)^2,
\end{align*}
%
i.e.~the variance of $\bm{V}$ w.r.t.~$P(\cdot| s,a)$. This can be expressed using our matrix notation as follows
%
\begin{equation*}
\Var_{\bP}(\bm{V}) = \bm{P} (\bm{V}\circ\bm{V})-(\bm{P} \bm{V})\circ(\bm{P} \bm{V}).
\end{equation*} 
%
Similarly, for any given policy $\pi$ we define 
%
\begin{equation*}
	\Var_{\bP_{\pi}}(\bm{V}) =  \bm{\Pi}^{\pi} \Var_{\bP}(\bm{V}) = \bm{P}_{\pi} (\bm{V}\circ\bm{V})-(\bm{P}_{\pi} \bm{V})\circ(\bm{P}_{\pi} \bm{V}) \in \mathbb{R}^{|\mathcal{S}|}.
\end{equation*} 
%

We shall also define $\widehat{\bm{V}}^{\pi}$, $\widehat{\bm{Q}}^{\pi}$, $\widehat{\bm{V}}^{\star}$, $\widehat{\bm{Q}}^{\star}$, $\widehat{\bm{P}}$, $\widehat{\bm{P}}^{\pi}$, $\widehat{\bm{P}}_{\pi}$,  $\Var_{\widehat{\bP}}(\bm{V})$, $\Var_{\widehat{\bP}_{\pi}}(\bm{V})$ w.r.t.~the empirical MDP $\widehat{\mathcal{M}}$ in an analogous fashion. 




==> proof-VR.tex <==
\section{Proof of Theorem~\ref{thm:main-asyn-VR-Q-learning}}



First we find it useful to write the Q-learning with variance reduction steps in terms of the matrix
form, where for notational clarity, we invoke some of the definitions that were used before. 
First recall definition $\bm{\Lambda}_{t}$ and $\bm{P}_{t}$ that are defined as in \eqref{eq:defn-Lambda-t}
and \eqref{eq:defn-Pt} respectively. 
\begin{align}
\bm{Q}_{t}=\big(\bm{I}-\bm{\Lambda}_{t}\big)\bm{Q}_{t-1}+\bm{\Lambda}_{t}\big(\bm{r} + \gamma\bm{P}_{t}\bm{V}_{t-1}\big
- \gamma \bm{P}_{t} \Vbar + \gamma \Ptil \Vbar)
\end{align}











